Rethinking Attention with Performers

We introduce Performers, Transformer architectures which can estimate regular (softmax) full-rank-attention Transformers with provable accuracy, but using only linear (as opposed to quadratic) space and time complexity, without relying on any priors such as sparsity or low-rankness. To approximate softmax attention-kernels, Performers use a novel Fast Attention Via positive Orthogonal Random features approach (FAVOR+), which may be of independent interest for scalable kernel methods. FAVOR+ can be also used to efficiently model kernelizable attention mechanisms beyond softmax. This representational power is crucial to accurately compare softmax with other kernels for the first time on large-scale tasks, beyond the reach of regular Transformers, and investigate optimal attention-kernels. Performers are linear architectures fully compatible with regular Transformers and with strong theoretical guarantees: unbiased or nearly-unbiased estimation of the attention matrix, uniform convergence and low estimation variance. We tested Performers on a rich set of tasks stretching from pixel-prediction through text models to protein sequence modeling. We demonstrate competitive results with other examined efficient sparse and dense attention methods, showcasing effectiveness of the novel attention-learning paradigm leveraged by Performers.

==> Performers - Fast Transformers V5/acknowledgements.tex <==
\section{Acknowledgements}
We thank Nikita Kitaev and Wojciech Gajewski for multiple discussions on the Reformer, and also thank Aurko Roy and Ashish Vaswani for multiple discussions on the Routing Transformer. We further thank Joshua Meier, John Platt, and Tom Weingarten for many fruitful discussions on biological data and useful comments on this draft. We lastly thank Yi Tay and Mostafa Dehghani for discussions on comparing baselines.

Valerii Likhosherstov acknowledges support from the Cambridge Trust and DeepMind. Lucy Colwell acknowledges support from the Simons Foundation. Adrian Weller acknowledges support from %the David MacKay Newton research fellowship at Darwin College,
a Turing AI Fellowship under grant EP/V025379/1, The Alan Turing Institute under EPSRC grant EP/N510129/1 and U/B/000074, and the Leverhulme Trust via CFI. 

==> Performers - Fast Transformers V5/algorithm.tex <==
\section{FAVOR+ Mechanism \& Positive Orthogonal Random Features}
\label{sec:algorithm}
Below we describe in detail the FAVOR+ mechanism - the backbone of the $\mathrm{Performer's}$ architecture. We introduce a new method for estimating softmax (and Gaussian) kernels with $\textbf{positive}$ orthogonal random features which FAVOR+ leverages for the robust and unbiased estimation of regular (softmax) attention and show how FAVOR+ can be applied for other attention-kernels.

\subsection{Preliminaries - regular attention mechanism}

Let $L$ be the size of an input sequence of tokens. Then regular dot-product attention \citep{transformer} is a mapping which accepts matrices $\mathbf{Q}, \mathbf{K}, \mathbf{V} \in \mathbb{R}^{L \times d}$ as input where $d$ is the hidden dimension (dimension of the latent representation). Matrices $\mathbf{Q}, \mathbf{K}, \mathbf{V}$ are intermediate representations of the input and their rows can be interpreted as \textit{queries}, \textit{keys} and \textit{values} of the continuous dictionary data structure respectively. \textit{Bidirectional (or non-directional \citep{bert}) dot-product attention} has the following form, where  $\mathbf{A} \in \mathbb{R}^{L \times L}$ is the so-called \textit{attention matrix}:
%\begin{gather}
\begin{equation}
\label{eq:attnorm}
    \mathrm{Att}_\leftrightarrow (\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \mathbf{D}^{-1} \mathbf{A} \mathbf{V}, \quad %\label{eq:att} \\
    \mathbf{A} = \exp ( \mathbf{Q} \mathbf{K}^\top / \sqrt{d}), \quad \mathbf{D} = \mathrm{diag} ( \mathbf{A} \mathbf{1}_L ). 
\end{equation}    
%\end{gather}
Here $\exp (\cdot)$ is applied elementwise, $\mathbf{1}_L$ is the all-ones vector of length $L$, and $\mathrm{diag} (\cdot)$ is a diagonal matrix with the input vector as the diagonal. Time and space complexity of computing (\ref{eq:attnorm}) are $O(L^2 d)$ and $O(L^{2}+Ld)$ respectively, because $\mathbf{A}$ has to be stored explicitly. Hence, in principle, dot-product attention of type (\ref{eq:attnorm}) is incompatible with end-to-end processing of long sequences. Bidirectional attention is applied in encoder self-attention and encoder-decoder attention in Seq2Seq architectures.

Another important type of attention is \textit{unidirectional dot-product attention} which has the form:
%\begin{gather}
\begin{equation}
    \mathrm{Att}_\to (\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \widetilde{\mathbf{D}}^{-1} \widetilde{\mathbf{A}} \mathbf{V}, \quad %\label{eq:uatt} \\
    \widetilde{\mathbf{A}} = \mathrm{tril} (\mathbf{A}), \quad \widetilde{\mathbf{D}} = \mathrm{diag} ( \widetilde{\mathbf{A}} \mathbf{1}_L ) , \label{eq:uattnorm}
\end{equation}
%\end{gather}
where $\mathrm{tril}(\cdot)$ returns the lower-triangular part of the argument matrix including the diagonal. As discussed in \citep{transformer}, unidirectional attention is used for autoregressive generative modelling, e.g. as self-attention in generative Transformers as well as the decoder part of Seq2Seq Transformers.

We will show that attention matrix $\mathbf{A}$ can be approximated up to any precision in time $O (L d^2\log(d))$. For comparison, popular methods leveraging sparsity via Locality-Sensitive Hashing (LSH) techniques \citep{reformer} have $O(L d^2 \log L)$ time complexity. 
In the main body of the paper we will describe FAVOR+ for bidirectional attention. Completely analogous results can be obtained for the unidirectional variant via the mechanism of \textit{prefix-sums} (all details in the Appendix \ref{subsec:unidirectional}).

\subsection{Generalized Kernelizable Attention}
\label{sec:gka}

FAVOR+ works for attention blocks using matrices $\mathbf{A} \in \mathbb{R}^{L \times L}$ of the form $\mathbf{A}(i,j) = \mathrm{K}(\mathbf{q}_{i}^{\top},\mathbf{k}_{j}^{\top})$, with $\mathbf{q}_{i}/\mathbf{k}_{j}$ standing for the $i^{th}/j^{th}$ query/key row-vector in $\mathbf{Q}/\mathbf{K}$ and kernel $\mathrm{K}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}_{+}$ defined for the (usually randomized) mapping: $\phi: \mathbb{R}^{d} \rightarrow \mathbb{R}_{+}^{r}$ (for some $r >0$) as:
\begin{equation}
\label{kernel-def}
\mathrm{K}(\mathbf{x}, \mathbf{y}) = \mathbb{E}[\phi(\mathbf{x})^{\top}\phi(\mathbf{y})].
\end{equation}
We call $\phi(\mathbf{u})$ a \textit{random feature map} for $\mathbf{u} \in \mathbb{R}^{d}$. 
For $\mathbf{Q}^{\prime},\mathbf{K}^{\prime} \in \mathbb{R}^{L \times r}$ with rows given as $\phi(\mathbf{q}_{i}^{\top})^{\top}$ and $\phi(\mathbf{k}_{i}^{\top})^{\top}$ respectively,
Equation \ref{kernel-def} leads directly to the efficient attention mechanism of the form:
\begin{equation}
    \widehat{\mathrm{Att}_\leftrightarrow} (\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \widehat{\mathbf{D}}^{-1} (\mathbf{Q}^{\prime}((\mathbf{K}^{\prime})^{\top} \mathbf{V})), \quad %\label{eq:att} \\
    \quad \widehat{\mathbf{D}} = \mathrm{diag} (\mathbf{Q}^{\prime}((\mathbf{K}^{\prime})^{\top} \mathbf{1}_L) ). 
\end{equation} 
Here $\widehat{\mathrm{Att}_\leftrightarrow}$ stands for the approximate attention and brackets indicate the order of computations. It is easy to see that such a mechanism is characterized by space complexity $O(Lr + Ld + rd)$ and time complexity $O(Lrd)$ as opposed to $O(L^{2}+Ld)$ and $O(L^{2}d)$ of the regular attention (see also Fig. \ref{fig:avqk}).
\vspace{-2mm}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.99\textwidth]{img/avqk.png}
  \caption{\small{Approximation of the regular attention mechanism $\mathbf{AV}$ (before $\mathbf{D}^{-1}$-renormalization) via (random) feature maps. Dashed-blocks indicate order of computation with corresponding time complexities attached.}}
  \label{fig:avqk}
\end{figure}

The above scheme constitutes the FA-part of the FAVOR+ mechanism. The remaining OR+ part answers the following questions: \textbf{(1)} How expressive is the attention model defined in Equation \ref{kernel-def}, and in particular, can we use it in principle to approximate regular softmax attention ? \textbf{(2)} How do we implement it robustly in practice, and in particular, can we choose $r \ll L$ for $L \gg d$ to obtain desired space and time complexity gains? We answer these questions in the next sections.

\subsection{How to and how not to approximate softmax-kernels for Attention}
\label{howto}

It turns out that by taking $\phi$ of the following form
for functions $f_{1},...,f_{l}:\mathbb{R} \rightarrow \mathbb{R}$,
function $g:\mathbb{R}^{d} \rightarrow \mathbb{R}$ and deterministic vectors $\omega_{i}$ or $\omega_{1},...,\omega_{m} \overset{\mathrm{iid}}{\sim} \mathcal{D}$ for some distribution $\mathcal{D} \in \mathcal{P}(\mathbb{R}^{d})$:
\begin{equation} \label{eq:feature}
\phi(\mathbf{x}) = \frac{h(\mathbf{x})}{\sqrt{m}}
(f_{1}(\omega_{1}^{\top}\mathbf{x}),...,f_{1}(\omega_{m}^{\top}\mathbf{x}),...,f_{l}(\omega_{1}^{\top}\mathbf{x}),...,f_{l}(\omega_{m}^{\top}\mathbf{x})),    
\end{equation}

we can model most kernels used in practice. Furthermore, in most cases $\mathcal{D}$ is isotropic (i.e. with pdf function constant on a sphere), usually Gaussian. For example, by taking $h(\mathbf{x})=1$, $l=1$ and $\mathcal{D}=\mathcal{N}(0,\mathbf{I}_{d})$ we obtain estimators of the so-called PNG-kernels \citep{unreas} (e.g. $f_{1} = \mathrm{sgn}$ corresponds to the angular kernel).
Configurations: $h(\mathbf{x})=1$, $l=2$, $f_{1}=\sin$, $f_{2}=\cos$ correspond to shift-invariant kernels, in particular $\mathcal{D}=\mathcal{N}(0, \mathbf{I}_{d})$ leads to the Gaussian kernel $\mathrm{K}_{\mathrm{gauss}}$ \citep{fourierapprox}. The \textit{softmax-kernel} which defines regular attention matrix $\mathbf{A}$ is given as:
\vspace{-0.75mm}
\begin{equation}
\mathrm{SM}(\mathbf{x}, \mathbf{y}) \overset{\mathrm{def}}{=} \exp(\mathbf{x}^{\top}\mathbf{y}).    
\end{equation}
In the above, without loss of generality, we omit $\sqrt{d}$-renormalization since we can equivalently renormalize input keys and queries. Since: $\mathrm{SM}(\mathbf{x}, \mathbf{y}) = \exp(\frac{\|\mathbf{x}\|^{2}}{2})\mathrm{K}_{\mathrm{gauss}}(\mathbf{x},\mathbf{y})\exp(\frac{\|\mathbf{y}\|^{2}}{2})$, based on what we have said, we obtain random feature map unbiased approximation of $\mathrm{SM}(\mathbf{x}, \mathbf{y})$ using trigonometric functions with: $h(\mathbf{x})=\exp(\frac{\|\mathbf{x}\|^{2}}{2})$, $l=2$, $f_{1}=\sin$, $f_{2}=\cos$. We call it $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}(\mathbf{x}, \mathbf{y})$. 

There is however a caveat there. The attention module from (\ref{eq:attnorm}) constructs for each token, a convex combination of value-vectors with coefficients given as corresponding renormalized kernel scores. That is why kernels producing non-negative scores are used. Applying random feature maps with potentially negative dimension-values ($\sin/\cos$) leads to unstable behaviours, especially when kernel scores close to $0$ (which is the case for many %lots of 
entries of $\mathbf{A}$ corresponding to low relevance tokens) are approximated by estimators with large variance in such regions. This results in abnormal behaviours, e.g. negative-diagonal-values renormalizers $\mathbf{D}^{-1}$, and consequently either completely prevents training or leads to sub-optimal models. 
We demonstrate empirically that this is what happens for $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}$ and provide detailed theoretical explanations showing that the variance of $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}$ is large as approximated values tend to $0$ (see: Section \ref{sec:theory}). This is one of the main reasons why the robust random feature map mechanism for approximating regular softmax attention was never proposed.

We propose a robust mechanism in this paper. Furthermore, the variance of our new unbiased positive random feature map estimator tends to $0$ as approximated values tend to $0$ (see: Section \ref{sec:theory}).

\begin{lemma}[Positive Random Features (PRFs) for Softmax]
\label{pos_random_features_lemma}
For $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$, $\mathbf{z}=\mathbf{x}+\mathbf{y}$ we have:
\begin{equation}
\label{main_eq}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = 
\mathbb{E}_{\omega \sim \mathcal{N}(0,\mathbf{I}_{d})}\!\Big[\mathrm{exp}\!\Big(\omega^{\top}\mathbf{x} - \frac{\|\mathbf{x}\|^{2}}{2}\Big)\mathrm{exp}\!\Big(\omega^{\top}\mathbf{y}-\frac{\|\mathbf{y}\|^{2}}{2}\Big)\Big]
=\Lambda \mathbb{E}_{\omega \sim \mathcal{N}(0,\mathbf{I}_{d})}\cosh(\omega^{\top}\mathbf{z}),
\end{equation}
where $\Lambda=\exp(-\frac{\|\mathbf{x}\|^{2}+\|\mathbf{y}\|^{2}}{2})$ and $\cosh$ is hyperbolic cosine. Consequently, softmax-kernel admits a positive random feature map unbiased approximation with  $h(\mathbf{x})=\exp(-\frac{\|\mathbf{x}\|^{2}}{2})$, $l=1$, $f_{1}=\exp$ and $\mathcal{D}=\mathcal{N}(0, \mathbf{I}_{d})$ or: $h(\mathbf{x})=\frac{1}{\sqrt{2}}\exp(-\frac{\|\mathbf{x}\|^{2}}{2})$, $l=2$, $f_{1}(u)=\exp(u)$, $f_{2}(u)=\mathrm{exp}(-u)$ and the same $\mathcal{D}$ (the latter for further variance reduction).
We call related estimators: $\widehat{\mathrm{SM}}^{+}_{m}$ and $\widehat{\mathrm{SM}}^{\mathrm{hyp+}}_{m}$.
\end{lemma}
% utility-final.png
\begin{figure}[h]
  \centering
  \includegraphics[width=0.99\textwidth]{img/utility-final2.png}
  \caption{\small{\textbf{Left:} Symmetrized (around origin) utility function $r$ (defined as the ratio of the mean squared errors (MSEs) of estimators built on: trigonometric and positive random features) as a function of the angle $\phi$ (in radians) between input feature vectors and their lengths $l$. Larger values indicate regions of $(\phi,l)$-space with better performance of positive random features. We see that for critical regions with $\phi$ large enough (small enough softmax-kernel values) our method is arbitrarily more accurate than trigonometric random features. Plot presented for domain $[-\pi, \pi] \times [-2, 2]$.} \textbf{Right:} The slice of function $r$ for fixed $l=1$ and varying angle $\phi$. \textbf{Right Upper Corner:} Comparison of the MSEs of both the estimators in a low softmax-kernel value region.\\}
  \label{fig:tower-function}
\end{figure}
In Fig. \ref{fig:tower-function} we visualize the advantages of positive versus standard trigonometric random features. In critical regions, where kernel values are small and need careful approximation, our method outperforms its counterpart. In Section \ref{sec:experiments} we further confirm our method's advantages empirically, using positive features to efficiently train softmax-based linear Transformers.
If we replace in (\ref{main_eq}) $\omega$ with $\sqrt{d}\frac{\omega}{\|\omega\|}$, we obtain the so-called \textbf{regularized softmax-kernel} $\mathrm{SMREG}$ which we can approximate in a similar manner, simply changing $\mathcal{D}=\mathcal{N}(0,\mathbf{I}_{d})$ to $\mathcal{D} = \mathrm{Unif}(\sqrt{d}\mathcal{S}^{d-1})$, a distribution corresponding to Haar measure on the sphere of radius $\sqrt{d}$ in $\mathbb{R}^{d}$, obtaining estimator $\widehat{\mathrm{SMREG}}^{+}_{m}$. As we show in Section \ref{sec:theory}, such random features can also be used to accurately approximate regular softmax-kernel.

\subsection{Orthogonal Random Features (ORFs)}
The above constitutes the R+ part of the FAVOR+ method. It remains to explain the O-part. To further reduce the variance of the estimator (so that we can use an even smaller number of random features $r$), we entangle different random samples $\omega_{1},...,\omega_{m}$ to be \textbf{exactly} orthogonal. This can be done while maintaining unbiasedness whenever isotropic distributions $\mathcal{D}$ are used (i.e. in particular in all kernels we considered so far) by the standard Gram-Schmidt orthogonalization procedure (see \citep{unreas} for details). ORFs is a well-known method, yet it turns out that it works particularly well with our introduced PRFs for softmax. This leads to the \textbf{first theoretical results} showing that ORFs can be applied to reduce the variance of softmax/Gaussian kernel estimators \textbf{for any} dimensionality $d$ rather than just asymptotically for large enough $d$ (as is the case for previous methods, see: next section) and leads to the \textbf{first exponentially small bounds} on large deviations probabilities that are strictly smaller than for non-orthogonal methods. Positivity of random features plays a key role in these bounds. The ORF mechanism requires $m \leq d$, but this will be the case in all our experiments. The pseudocode of the entire FAVOR+ algorithm is given in Appendix \ref{appendix:main_algorithm}.

Our theoretical results are tightly aligned with experiments. We show in Section \ref{sec:experiments} that PRFs+ORFs drastically improve accuracy of the approximation of the attention matrix and enable us to reduce $r$ which results in an accurate as well as space and time efficient mechanism which we call FAVOR+.





==> Performers - Fast Transformers V5/broader_impact.tex <==
\section{Broader impact}
\label{sec:broader_impact}
We believe that the presented algorithm can be impactful in various ways:

\textbf{Biology and Medicine:} Our method has the potential to directly impact research on biological sequence analysis by enabling the Transformer to be applied to much longer sequences without constraints on the structure of the attention matrix. The initial application that we consider is the prediction of interactions between proteins on the proteome scale. Recently published approaches require large evolutionary sequence alignments, a bottleneck for applications to mammalian genomes \citep{cong2019protein}. The potentially broad translational impact of applying these approaches to biological sequences was one of the main motivations of this work. We believe that modern bioinformatics can immensely benefit from new machine learning techniques with Transformers being among the most promising. Scaling up these methods to train faster more accurate language models opens the door to the ability to design sets of molecules with pre-specified interaction properties. These approaches could be used to augment existing physics-based design strategies that are of critical importance for example in the development of new nanoparticle vaccines \citep{marcandalli2019induction}.  

\textbf{Environment:} As we have shown, Performers with FAVOR+ are characterized by much lower compute costs and substantially lower space complexity which can be directly translated to $\mathrm{CO}_{2}$ emission reduction \citep{co2} and lower energy consumption \citep{energy}, as regular Transformers require very large computational resources.

\textbf{Research on Transformers:} We believe that our results can shape research on efficient Transformers architectures, guiding the field towards methods with strong mathematical foundations. Our research may also hopefully extend Transformers also beyond their standard scope (e.g. by considering the Generalized Attention mechanism and connections with kernels). Exploring scalable Transformer architectures that can handle $L$ of the order of magnitude few thousands and more, preserving accuracy of the baseline at the same time, is a gateway to new breakthroughs in bio-informatics, e.g. language modeling for proteins, as we explained in the paper. Our presented method can be potentially a first step.

\textbf{Backward Compatibility:} Our Performer can be used on the top of a regular pre-trained Transformer as opposed to other Transformer variants. Even if up-training is not required, FAVOR+ can still be used for fast inference with no loss of accuracy. We think about this backward compatibility as a very important additional feature of the presented techniques that might be particularly attractive for practitioners.

\textbf{Attention Beyond Transformers:} Finally, FAVOR+ can be applied to approximate exact attention also outside the scope of Transformers. This opens a large volume of new potential applications including: hierarchical attention networks (HANS) \citep{hans}, graph attention networks \citep{gran}, image processing \citep{attention_cvpr}, and reinforcement learning/robotics \citep{tang}. 





==> Performers - Fast Transformers V5/conclusion.tex <==
\vspace{-3mm}
\section{Conclusion}
\label{sec:conclusion}
We presented $\mathrm{Performer}$, a new type of Transformer, relying on our Fast Attention Via positive Orthogonal Random features (FAVOR+) mechanism to significantly improve space and time complexity of regular Transformers. Our mechanism provides to our knowledge the first effective unbiased estimation of the original softmax-based Transformer with linear space and time complexity and opens new avenues in the research on Transformers and the role of non-sparsifying attention mechanisms.

%Our work opens many interesting avenues for future work. %One question to be explored is whether our performance %benefit is due to the inherent dense structure of the %attention patterns that need to be learned in these %applications, \textcolor{red}{or other factors such as the %potential negative effect of reversible layers (due to %forgetting) on the Reformer. }




==> Performers - Fast Transformers V5/experiments.tex <==
\vspace{-2.5mm}
\section{Experiments}
\label{sec:experiments}
We implemented our setup on top of pre-existing Transformer training code in Jax \citep{jax} optimized with just-in-time (\texttt{jax.jit}) compilation, and complement our theory with empirical evidence to demonstrate the practicality of FAVOR+ in multiple settings. Unless explicitly stated, a Performer replaces only the attention component with our method, while all other components are exactly the same as for the regular Transformer. For shorthand notation, we denote unidirectional/causal modelling as \textbf{(U)} and bidirectional/masked language modelling as \textbf{(B)}. 

In terms of baselines, we use other Transformer models for comparison, although some of them are restricted to only one case - e.g. Reformer \citep{reformer} is only (U), and Linformer \citep{linformer} is only (B). Furthermore, we use PG-19 \citep{compr} as an alternative (B) pretraining benchmark, as it is made for long-length sequence training compared to the (now publicly unavailable) BookCorpus \citep{bookcorpus} + Wikipedia dataset used in BERT \citep{bert} and Linformer. All model and tokenization hyperparameters are shown in Appendix \ref{appendix:hyperparameters}.

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{img/model_regular_opt.png}
  \caption{\small{Comparison of Transformer and Performer in terms of forward and backward pass speed and maximum $L$ allowed. "X" (OPT) denotes the maximum possible speedup achievable, when attention simply returns the $\mathbf{V}$-matrix. Plots shown up to when a model produces an out of memory error on a V100 GPU with 16GB. Vocabulary size used was 256. Best in color.}}
  \label{fig:backward_pass}
\end{figure}

\subsection{Computational costs}
We compared speed-wise the backward pass of the Transformer and the Performer in (B) setting, as it is one of the main computational bottlenecks during training, when using the regular default size $(n_{heads}, n_{layers}, d_{ff}, d) = (8,6,2048,512)$, where $d_{ff}$ denotes the width of the MLP layers. We observed (Fig. \ref{fig:backward_pass}) that in terms of $L$, the Performer reaches nearly linear time and sub-quadratic memory consumption (since the explicit $O(L^{2})$ attention matrix is not stored). In fact, the Performer achieves nearly optimal speedup and memory efficiency possible, depicted by the "X"-line when attention is replaced with the "identity function" simply returning the $\mathbf{V}$-matrix. The combination of both memory and backward pass efficiencies for large $L$ allows respectively, large batch training and lower wall clock time per gradient step. Extensive additional results are demonstrated in Appendix \ref{appendix:computation_costs_bidirectional} by varying layers, raw attention, and architecture sizes.

\subsection{Softmax attention approximation error}
\label{subsec:approx_error_compatibility}

We further examined the approximation error via FAVOR+ in Fig. \ref{fig:approx}.
%As already established in Sec. \ref{sec:theory} that convergence is independent of $L$, 
We demonstrate that \textbf{1.} Orthogonal features produce lower error than unstructured (IID) features, \textbf{2.} Positive features produce lower error than trigonometric $\sin$/$\cos$ features. These two empirically validate the PORF mechanism.
%\vspace{0.5mm}
\begin{figure}[H]
  \includegraphics[width=0.498\textwidth]{img/attention_output_ortho_iid.png}
  \includegraphics[width=0.498\textwidth]{img/attention_output_sin_exp.png}
  \caption{\small{MSE of the approximation output when comparing Orthogonal vs IID features and trigonometric $\sin$/$\cos$ vs positive features. We took $L = 4096, d = 16$, and varied the number of random samples $m$. Standard deviations shown across 15 samples of appropriately normalized random matrix input data.}}
  \label{fig:approx}
\end{figure}

To further improve overall approximation of attention blocks across multiple iterations which further improves training, random samples should be periodically redrawn (Fig. \ref{fig:backward_compatibility}, right). This is a cheap procedure, but can be further optimized (Appendix \ref{subsec:extensions}).

\subsection{Softmax approximation on Transformers}
\label{subsec:softmax_approx_transformer}

Even if the approximation of the attention mechanism is tight, small errors can easily propagate throughout multiple Transformer layers (e.g. MLPs, multiple heads), as we show in Fig. \ref{fig:appendix_approx} (Appendix). In other words, the model's \textit{Lipschitz constant} can easily scale up small attention approximation error, which means that very tight approximations may sometimes be needed. Thus, when applying FAVOR(+)'s softmax approximations on a Transformer model (i.e. "Performer-X-SOFTMAX"), we demonstrate that: 

\textbf{1.} Backwards compatibility with pretrained models is available as a benefit from softmax approximation, via small finetuning (required due to error propagation) even for trigonometric features (Fig. \ref{fig:backward_compatibility}, left) on the LM1B dataset \citep{lm1b}.
However, when on larger dataset PG-19, \textbf{2.} Positive (POS) softmax features (with redrawing) become crucial for achieving performance matching regular Transformers (Fig. \ref{fig:backward_compatibility}, right). 

\begin{figure}[H]
  \centering
  \includegraphics[width=0.99\textwidth]{img/softmax_plot.png}
  \caption{\small We transferred the original pretrained Transformer's weights into the Performer, which produces an initial non-zero 0.07 accuracy (dotted orange line), but quickly recovers accuracy in a small fraction of the original number of gradient steps. However on PG-19, Trigonometric (TRIG) softmax approximation becomes highly unstable (full curve in Appendix \ref{subsec:unstable_trig}), while positive features (POS) (without redrawing) and Linformer (which also approximates softmax) \textit{even with redrawn projections}, plateau at the same perplexity. Positive softmax with feature redrawing is necessary to match the Transformer, with SMREG (regularization from Sec. \ref{ort-theorem}) allowing faster convergence. Additional ablation studies over many attention kernels, showing also that trigonometric random features lead even to NaN values in training are given in Appendix \ref{subsec:appendix_generalized_attention}.}
  \label{fig:backward_compatibility}
\end{figure}

\subsection{Multiple layer training for proteins}
We further benchmark the Performer on both (U) and (B) cases by training a 36-layer model using protein sequences from the Jan. 2019 release of TrEMBL \citep{uniprot2019uniprot}, similar to \citep{progen}. In Fig. \ref{fig:big_benchmarking}, the Reformer and Linformer \textit{significantly drop in accuracy} on the protein dataset. Furthermore, the usefulness of generalized attention is evidenced by Performer-RELU (taking $f=\mathrm{ReLU}$ in Equation \ref{eq:feature}) achieving the highest accuracy in both (U) and (B) cases. Our proposed softmax approximation is also shown to be tight, achieving the same accuracy as the exact-softmax Transformer and confirming our theoretical claims from Section \ref{sec:theory}. 

\begin{figure}[H]
  \centering
  \includegraphics[width=1.0\textwidth]{img/protein_both.png}
  \caption{\small Train = Dashed, Validation = Solid. For TrEMBL, we used the exact same model parameters $(n_{heads}, n_{layers}, d_{ff}, d)  = (8, 36, 1024, 512)$ from \protect\citep{progen} for all runs. For fairness, all TrEMBL experiments used 16x16 TPU-v2's. Batch sizes were maximized for each separate run given the compute constraints. Hyperparameters can be found in Appendix \ref{appendix:hyperparameters}. Extended results including dataset statistics, out of distribution evaluations, and visualizations, can be found in Appendix \ref{appendix:protein_extended}.}
  \label{fig:big_benchmarking}
\end{figure}
\vspace{-2mm}
\subsection{Large length training - Common datasets}
On the standard (U) ImageNet64 benchmark from \citep{parmar} with $L = 12288$ which is unfeasible for regular Transformers, we set all models to use the same $(n_{heads}, d_{ff}, d)$ but varying $n_{layers}$. Performer/6-layers matches the Reformer/12-layers, while the Performer/12-layers matches the Reformer/24-layers (Fig. \ref{fig:im64_protein_8192}: left). Depending on hardware (TPU or GPU), we also found that the Performer can be 2x faster than the Reformer via Jax optimizations for the (U) setting. 

For a proof of principle study, we also create an initial protein benchmark for predicting interactions among groups of proteins by concatenating protein sequences to length $L = 8192$ from TrEMBL, long enough to model protein interaction networks without the large sequence alignments required by existing methods \citep{cong2019protein}. In this setting, a regular Transformer overloads memory even at a batch size of $1$ per chip, by a wide margin. Thus as a baseline, we were forced to use a significantly smaller variant, reducing to $(n_{heads}, n_{layers}, d_{ff}, d) = (8, \{1,2,3\}, 256, 256)$. Meanwhile, the Performer trains efficiently at a batch size of 8 per chip using the standard $(8, 6, 2048, 512)$ architecture. We see in Fig. \ref{fig:im64_protein_8192} (right subfigure) that the smaller Transformer ($n_{layer} = 3$) is quickly bounded at $\approx 19\%$, while the Performer is able to train continuously to $\approx 24\%$.
%ImageNet64 results are also presented in Fig. \ref{fig:im64_protein_8192}.

\begin{figure}[H]
  \centering
  \includegraphics[width=1.0\textwidth]{img/im64_concat_protein.png}
  \caption{\small Train = Dashed, Validation = Solid. For ImageNet64, all models used the standard $(n_{heads}, d_{ff}, d) = (8, 2048, 512)$. We further show that our positive softmax approximation achieves the same performance as ReLU in Appendix \ref{subsec:softmax_unidirectional}. For concatenated TrEMBL, we varied $n_{layers} \in \{1,2,3\}$ for the smaller Transformer. Hyperparameters can be found in Appendix \ref{appendix:hyperparameters}.}
  \label{fig:im64_protein_8192}
\end{figure}









==> Performers - Fast Transformers V5/intro_related_work.tex <==
\section{Introduction and related work}
\label{sec:intro_related_work}

Transformers \citep{transformer, universal_t} are powerful neural network architectures that have become SOTA in several areas of machine learning including natural language processing (NLP) (e.g. speech recognition \citep{luo}), neural machine translation (NMT) \citep{nmt}, document generation/summarization, time series prediction, generative modeling (e.g. image generation \citep{parmar}), music generation \citep{simon}, and bioinformatics \citep{rives, progen, ingraham2019generative, elnaggar2019end, du2020energy}. 

Transformers rely on a trainable \textit{attention} mechanism that identifies complex dependencies between the elements of each input sequence. Unfortunately, the regular Transformer scales quadratically with the number of tokens $L$ in the input sequence, which is prohibitively expensive for large $L$ and precludes its usage in settings with limited computational resources even for moderate values of $L$. 
Several solutions have been proposed to address this issue \citep{longformer, conformer, imputer, sparsetr, image_transformer}. Most approaches restrict the attention mechanism to attend to local neighborhoods \citep{parmar} or incorporate structural priors on attention such as sparsity \citep{sparsetr}, pooling-based compression \citep{compr} clustering/binning/convolution techniques (e.g. \citep{routing_t} which applies $k$-means clustering to learn dynamic sparse attention regions, or \citep{reformer}, where locality sensitive hashing is used to group together tokens of similar embeddings), sliding windows \citep{longformer}, or truncated targeting \citep{chelba}. 
There is also a long line of research on using dense attention matrices, but defined by low-rank kernels
substituting softmax \citep{trans-rnns, shen}. Those methods critically rely on kernels admitting explicit representations as dot-products of finite positive-feature vectors.

The approaches above do not aim to approximate regular attention, but rather propose simpler and more tractable attention mechanisms, often by incorporating additional constraints (e.g. identical query and key sets as in \citep{reformer}), or by trading regular with sparse attention using more layers \citep{sparsetr}. Unfortunately, there is a lack of rigorous guarantees for the representation power produced by such methods, and sometimes the validity of sparsity patterns can only be verified empirically through trial and error by constructing special GPU operations (e.g. either writing C++ CUDA kernels \citep{sparsetr} or using TVMs \citep{longformer}). Other techniques %improving 
which aim to reduce %overall 
Transformers' space complexity include reversible residual layers allowing one-time activation storage in training \citep{reformer} and shared attention weights \citep{shared_weights}. These constraints may impede application %of the Transformer 
to long-sequence problems, where approximations of the attention mechanism are not sufficient. Approximations based on truncated back-propagation \citep{transformerxl} are also unable to capture long-distance correlations since the gradients are only propagated inside a localized window.
Other methods propose biased estimation of %the 
regular attention but only in the non-causal setting and with large mean squared error \citep{linformer}.

%Other methods propose algorithms that
%in principle can provide estimation (yet not %unbiased) of the regular attention, but are not %feasible in practice due to inherent difficulty %of approximating regular non-Lipschitz  %attention (e.g. require projection matrices %with entries of magnitude $2^{-100}$ for %$100$-dimensional problems, see: Theorem 2 in %\citep{linformer}). Those methods are applied %by severely relaxing the structure of the %original algorithms, leading to mechanisms no %longer approximating regular attention (see: %Section \ref{sec:experiments}).

In response, we introduce the first Transformer architectures, \textit{Performers}, capable of \textbf{provably} accurate and practical estimation of regular (softmax) full-rank attention, but of only linear space and time complexity and \textbf{not relying on any priors} such as sparsity or low-rankness. Performers use the \textit{Fast Attention Via positive Orthogonal Random features} (FAVOR+) mechanism, leveraging new methods for approximating softmax and Gaussian kernels, which we propose. We believe these methods are of independent interest, contributing to the theory of scalable kernel methods. 
Consequently, Performers are the first linear architectures \textbf{fully compatible} (via small amounts of fine-tuning) with regular Transformers, providing strong theoretical guarantees: unbiased or nearly-unbiased estimation of the attention matrix, uniform convergence and lower variance of the approximation.

%Importantly, 
FAVOR+ can be also applied to efficiently model other kernelizable attention mechanisms beyond softmax. This representational power is crucial to accurately compare softmax with other kernels for the first time on large-scale tasks, that are beyond the reach of regular Transformers, and find for them optimal attention-kernels.
FAVOR+ can also be applied beyond the Transformer scope as a more scalable replacement for regular attention, which itself has a wide variety of uses in computer vision \citep{attention_cvpr}, reinforcement learning \citep{relational}, training with softmax cross entropy loss, and even combinatorial optimization \citep{pointer}.

We test Performers on a rich set of tasks ranging from pixel-prediction through text models to protein sequence modeling. We demonstrate competitive results with other examined efficient sparse and dense attention methods, showcasing the effectiveness of the novel attention-learning paradigm leveraged by Performers. We emphasize that in principle, FAVOR+ can also be combined with other techniques, such as reversible layers \citep{reformer} or cluster-based attention \citep{routing_t}. 





 





==> Performers - Fast Transformers V5/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Performers - Fast Transformers V5/rebuttal.tex <==
\newpage
\section*{Rebuttal (Temporary Section)}

\subsection*{R.1 Comparison with Linear Transformer}
We use the attention implementation of the Linear Transformer from \citep{trans-rnns}, which mainly involves setting our feature map $\phi(x) = \text{elu}(x) + 1$, where $\text{elu}(x)$ is the shifted-eLU function from \citep{elu}. For the sake of fairness and to prevent confounding results, while \citep{trans-rnns} also uses the GeLU nonlinearity for the MLPs in the Linear Transformer, we instead use the original ReLU nonlinearity. We also used the exact same training hyperparameters as Performer-ReLU. Ultimately, we empirically found that the Linear Transformer possessed numerical instability during training via unstable training curves, \textbf{ultimately stopping training by producing exploding gradients (NaNs)} (Fig. R1).

\begin{figure}[h]
  \centering
  \includegraphics[width=0.99\textwidth]{img/linear_transformer_kernel_on.png}
  \caption*{\small{Fig. R1: \textbf{Left:} In the unidirectional 36-ProGen setting, we ran 3 seeds of the Linear Transformer, and found that all 3 seeds produced exploding gradients very early on, stopping the training run. \textbf{Right:} The Linear Transformer in the bidirectional setting also produced an exploding gradient in the middle of training, near 125K steps. Exploding gradients can be evidenced by the sharp drop in train accuracy right before a NaN error.}}
  \label{fig:rebuttal_linear_trans}
\end{figure}

\subsection*{R.2 Long Range Arena Paper Results (\textcolor{blue}{\url{https://arxiv.org/abs/2011.04006}})}
\vspace{-2mm}
We present here the comparison of Performers with several other architectures conducted in the paper: \textit{Long Range Arena: A Benchmark for Efficient Transformers} (`LRA'). %-paper)
Performers are compared against many additional (scalable and not scalable) methods not included in our submission: \textit{Local Attention}, \textit{Sparse Attention}, \textit{Longformer}, \textit{Sinkhorn Transformer}, \textit{Synthesizer}, \textit{Big Bird} and the aforementioned \textit{Linear Transformer} on challenging long range context tasks. Performers obtain the largest LRA (Long Range Arena) score among all tested \textbf{scalable} Transformers methods (which we define by having speed of > 100 examples/sec). Tasks used for comparison include: \textbf{(1)} a longer variation of the standard ListOps task proposed in \citep{listops}, \textbf{(2)} byte-level text classification using real-world data, \textbf{(3)} byte-level document retrieval, \textbf{(4)} image classification on sequences of pixels, and \textbf{(5)} Pathfinder task (long-range spatial dependency problem).
\vspace{0.1cm}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.99\textwidth]{img/lra-all-3.pdf}
  \vspace{0.15cm}
  \caption*{\small{Fig. R2 (From LRA-paper): \textbf{Upper Table:} Results on Long-Range Arena benchmark. Best model is in boldface and second best is underlined. All models do not learn anything on Path-X task, contrary to the Pathfinder task and this is denoted by FAIL. This shows that increasing the sequence length can cause seriously difficulties for model training. The authors leave Path-X on this benchmark for future challengers but do not include it on the average (Avg.) score as it has no impact on relative performance. \textbf{Lower Table:} Benchmark results of all X-former models with a consistent batch size of 32 across all models. The authors report relative speed increase/decrease in comparison with the vanilla Transformer in brackets besides the steps per second. Memory usage refers to per device memory usage across each TPU device. Benchmarks are run on 4x4 TPU-v3 chips. \textbf{Right Fig:} Performance (y axis), speed (x axis), and memory footprint (size of the circles) of different
models.} }
  \label{fig:rebuttal_lra}
\end{figure}


==> Performers - Fast Transformers V5/theory.tex <==
\section{Theoretical results}
\label{sec:theory}

We present here the theory of positive orthogonal random features for softmax-kernel estimation. All these results can be applied also to the Gaussian kernel, since as explained in the previous section, one can be obtained from the other by renormalization (see: Section \ref{howto}).
All proofs and additional more general theoretical results with a discussion
are given in the Appendix.

\begin{lemma}[positive (hyperbolic) versus trigonometric random features]
\label{mse-lemma}
The following is true:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})) =
\frac{1}{2m} \exp(\|\mathbf{x}+\mathbf{y}\|^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})
(1-\mathrm{exp}(-\|\mathbf{x}-\mathbf{y}\|^{2}))^{2}, \\ 
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{m}\exp(\|\mathbf{x}+\mathbf{y}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{x}+\mathbf{y}\|^{2})),\\
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyp}+}_{m}(\mathbf{x}, \mathbf{y})) =
\frac{1}{2}(1-\exp(-\|\mathbf{x}+\mathbf{y}\|^{2}))\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})),
\end{split}
\end{align}
for independent random samples $\omega_{i}$, and where $\mathrm{MSE}$ stands for the mean squared error.
\end{lemma}
Thus, for $\mathrm{SM}(\mathbf{x}, \mathbf{y}) \rightarrow 0$ we have: $\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})) \rightarrow \infty$ and $\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})) \rightarrow 0$. Furthermore, the hyperbolic estimator provides additional accuracy improvements that are strictly better than those from $\widehat{\mathrm{SM}}_{2m}^{\mathrm{+}}(\mathbf{x}, \mathbf{y})$ with twice as many random features. The next result shows that the regularized softmax-kernel is in practice an accurate proxy of the softmax-kernel in attention.

\begin{theorem}[regularized versus softmax-kernel]
\label{reg-theorem}
Assume that the $L_{\infty}$-norm of the attention matrix for the softmax-kernel satisfies: $\|\mathbf{A}\|_{\infty} \leq C$ for some constant $C \geq 1$. Denote by $\mathbf{A}^{\mathrm{reg}}$ the corresponding attention matrix for the regularized softmax-kernel. The following holds:
\begin{equation}
\inf_{i,j} \frac{\mathbf{A}^{\mathrm{reg}}(i,j)}{\mathbf{A}(i, j)} \geq 1 - \frac{2}{d^{\frac{1}{3}}} + o\left(\frac{1}{d^{\frac{1}{3}}}\right), \textrm{ and } \sup_{i,j} \frac{\mathbf{A}^{\mathrm{reg}}(i,j)}{\mathbf{A}(i, j)} \leq 1. 
\end{equation}
Furthermore, the latter holds for $d \geq 2$ even if the $L_{\infty}$-norm condition is not satisfied, i.e. the regularized softmax-kernel is a universal lower bound for the softmax-kernel. 
\end{theorem}
Consequently, positive random features for $\mathrm{SMREG}$ can be used to approximate the softmax-kernel.
Our next result shows that orthogonality provably reduces mean squared error of the estimation with positive random features \textbf{for any dimensionality $d>0$} and we explicitly provide the gap.
\begin{theorem}
\label{var-theorem}
If $\widehat{\mathrm{SM}}_{m}^{\mathrm{ort+}}(\mathbf{x}, \mathbf{y})$ stands for the modification of
$\widehat{\mathrm{SM}}_{m}^{+}(\mathbf{x}, \mathbf{y})$ with orthogonal random features (and thus for $m \leq d$), then the following holds for any $d >0$:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}_{m}^{\mathrm{ort+}}(\mathbf{x}, \mathbf{y})) \leq 
\mathrm{MSE}(\widehat{\mathrm{SM}}_{m}^{+}(\mathbf{x}, \mathbf{y})) - \frac{2 (m - 1)}{m(d+2)}\left(\mathrm{SM}(\mathbf{x}, \mathbf{y}) - \exp\left(- \frac{\| \*x \|^2 + \| \*y \|^2}{2}\right) \right)^2.
\end{equation}
Furthermore, completely analogous result holds for the regularized softmax-kernel $\mathrm{SMREG}$.
\end{theorem}
For the regularized softmax-kernel, orthogonal features provide additional concentration results - the first exponentially small bounds for probabilities of estimators' tails that are strictly better than for non-orthogonal variants for every $d>0$. Our next result enables us to explicitly estimate the gap.

\begin{theorem}
\label{ort-theorem}
Let $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$. The following holds for any $a > \mathrm{SMREG}(\mathbf{x},\mathbf{y})$, $\theta > 0$ and $m \leq d$:
\begin{gather*}
    \mathbb{P}[\widehat{\mathrm{SMREG}}^{+}_{m}(\mathbf{x}, \mathbf{y}) > a] \leq \exp(-\theta m a) M_Z (\theta)^m, \quad \mathbb{P}[\widehat{\mathrm{SMREG}}^{\mathrm{ort+}}_{m}(\mathbf{x}, \mathbf{y}) > a] \\
    \leq \exp(-\theta m a) \biggl( M_Z (\theta)^m - \exp\left(-\frac{m}{2} (\| \*x \|^2 + \| \*y \|^2)\right) \frac{\theta^4 m (m - 1)}{4 (d + 2)} \| \*x + \*y \|^4 \biggr)
\end{gather*}
where $\widehat{\mathrm{SMREG}}^{\mathrm{ort+}}_{m}(\mathbf{x}, \mathbf{y})$ stands for the modification of $\widehat{\mathrm{SMREG}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})$ with ORFs, $X = \Lambda \exp(\sqrt{d}\frac{\omega^{\top}}{\|\omega\|_{2}}(\mathbf{x}+\mathbf{y}))$, $\omega \sim \mathcal{N}(0,\mathbf{I}_{d})$, $\Lambda$ is as in Lemma \ref{pos_random_features_lemma} and
$M_{Z}$ is the moment generating function of $Z$.
\end{theorem}

We see that ORFs provide exponentially small and sharper bounds for critical regions where the softmax-kernel is small. 
Below we show that even for the $\mathrm{SM}^{\mathrm{trig}}$ mechanism with ORFs, it suffices to take $m=\Theta(d\log(d))$ random projections to accurately approximate the attention matrix (thus if not attention renormalization, PRFs would not be needed). In general, $m$ depends on the dimensionality $d$ of the embeddings, radius $R$ of the ball where all queries/keys live and precision parameter $\epsilon$ (see: Appendix~\ref{sec:ball} for additional discussion), but does not depend on input sequence length $L$.

%So for a fixed maximum length $R$ of %queries/keys (see Appendix~\ref{sec:ball} %for a discussion of this restriction), the number of random projections $m$ required is a %function of data dimensionality $d$ and %precision parameter $\epsilon$. 

%PRFs improve on that by robustifying approximation of the renormalizer $\mathbf{D}^{-1}$ %from Eq. \ref{eq:attnorm}
\begin{theorem}[uniform convergence for attention approximation]
\label{thm:uniform}
Assume that $L_{2}$-norms of queries/keys are upper-bounded by $R>0$. Define $l=Rd^{-\frac{1}{4}}$ and take 
$h^{*} = \exp(\frac{l^{2}}{2})$.
Then for any $\epsilon>0$, $\delta=\frac{\epsilon}{(h^{*})^{2}}$
and the number of random projections $m=\Theta(\frac{d}{\delta^{2}}\log(\frac{4d^{\frac{3}{4}} R}{\delta}))$ the following holds for the attention approximation mechanism leveraging estimators $\widehat{\mathrm{SM}}^{\mathrm{trig}}$ with ORFs:
$\|\widehat{\mathbf{A}}-\mathbf{A}\|_{\infty} \leq \epsilon$ with any constant probability, where $\widehat{\mathbf{A}}$ approximates the attention matrix $\mathbf{A}$.
\end{theorem}








==> Performers - Fast Transformers V5/theory_old.tex <==

\section{Theoretical convergence analysis}
\label{sec:theory}
In contrast to other methods approximating the attention matrix $\mathbf{A}$, our algorithm provides provable strong uniform convergence theoretical guarantees for compact domains. We show that $M_{\mathrm{opt}}$, the optimal number of random features, does not depend on $L$ but only on $d$. In fact, we prove that if we take $M_{\mathrm{opt}} = \Theta(d\log(d))$, then with $O(L d^2\log(d))$-time, we can approximate $\mathbf{A}$ up to any precision, regardless of the number of tokens $L$. In order to provide those guarantees for FAVOR, we leverage recent research on the theory of negative dependence for ORFs \citep{Lin2020DemystifyingOM}.
The following is true:

\begin{theorem}[Uniform convergence of FAVOR]
\label{uniform_convergence}
Take the generalized attention mechanism defined by $g,h:\mathbb{R}^{d} \rightarrow \mathbb{R}$ (see: Sec. \ref{sec:generalized}) and a radial basis function (RBF) kernel \citep{geom} $K$ with corresponding spectral distribution $\Omega$ (e.g. Gaussian kernel for which $\Omega=\mathcal{N}(0,\mathbf{I}_{d})$). Assume that the rows of matrices $\mathbf{Q}$ and $\mathbf{K}$ are taken from a ball $B(R)$ of radius $R$, centered at $0$ (i.e. norms of queries and keys are upper-bounded by $R$). 
Define $l=Rd^{-\frac{1}{4}}$ and take $g^{*} = \max_{\mathbf{x} \in B(l)}|g(\mathbf{x})|$, $h^{*} = \max_{\mathbf{x} \in B(l)}|h(\mathbf{x})|$.
Then for any $\epsilon>0$, $\delta=\frac{\epsilon}{g^{*}h^{*}}$
and the number of random features $M = \Omega(\frac{d}{\delta^{2}}\log(\frac{4\sigma R}{\delta d^{\frac{1}{4}}}))$ for $\sigma=\mathbb{E}_{\omega \sim \Omega}[\omega^{\top}\omega]$ the following holds:
$
\|\widehat{\mathbf{A}}-\mathbf{A}\|_{1} \leq \epsilon     
$
with any constant probability,
where $\widehat{\mathbf{A}}$ approximates generalized attention matrix via FAVOR with R-ORFs. 
\end{theorem}

The result holds in particular for regular attention using Gaussian kernels (see: Sec. \ref{sec:generalized}) for which $M_{\mathrm{opt}}=\Omega(\frac{d}{\delta^{2}}\log(\frac{4d^{\frac{3}{4}} R}{\delta}))$ since $\sigma = d$.




==> rebuttal.tex <==
\newpage
\section*{Rebuttal (Temporary Section)}

\subsection*{R.1 Comparison with Linear Transformer}
We use the attention implementation of the Linear Transformer from \citep{trans-rnns}, which mainly involves setting our feature map $\phi(x) = \text{elu}(x) + 1$, where $\text{elu}(x)$ is the shifted-eLU function from \citep{elu}. For the sake of fairness and to prevent confounding results, while \citep{trans-rnns} also uses the GeLU nonlinearity for the MLPs in the Linear Transformer, we instead use the original ReLU nonlinearity. We also used the exact same training hyperparameters as Performer-ReLU. Ultimately, we empirically found that the Linear Transformer possessed numerical instability during training via unstable training curves, \textbf{ultimately stopping training by producing exploding gradients (NaNs)} (Fig. R1).

\begin{figure}[h]
  \centering
  \includegraphics[width=0.99\textwidth]{img/linear_transformer_kernel_on.png}
  \caption*{\small{Fig. R1: \textbf{Left:} In the unidirectional 36-ProGen setting, we ran 3 seeds of the Linear Transformer, and found that all 3 seeds produced exploding gradients very early on, stopping the training run. \textbf{Right:} The Linear Transformer in the bidirectional setting also produced an exploding gradient in the middle of training, near 125K steps. Exploding gradients can be evidenced by the sharp drop in train accuracy right before a NaN error.}}
  \label{fig:rebuttal_linear_trans}
\end{figure}

\subsection*{R.2 Long Range Arena Paper Results (\textcolor{blue}{\url{https://arxiv.org/abs/2011.04006}})}
\vspace{-2mm}
We present here the comparison of Performers with several other architectures conducted in the paper: \textit{Long Range Arena: A Benchmark for Efficient Transformers} (`LRA'). %-paper)
Performers are compared against many additional (scalable and not scalable) methods not included in our submission: \textit{Local Attention}, \textit{Sparse Attention}, \textit{Longformer}, \textit{Sinkhorn Transformer}, \textit{Synthesizer}, \textit{Big Bird} and the aforementioned \textit{Linear Transformer} on challenging long range context tasks. Performers obtain the largest LRA (Long Range Arena) score among all tested \textbf{scalable} Transformers methods (which we define by having speed of > 100 examples/sec). Tasks used for comparison include: \textbf{(1)} a longer variation of the standard ListOps task proposed in \citep{listops}, \textbf{(2)} byte-level text classification using real-world data, \textbf{(3)} byte-level document retrieval, \textbf{(4)} image classification on sequences of pixels, and \textbf{(5)} Pathfinder task (long-range spatial dependency problem).
\vspace{0.1cm}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.99\textwidth]{img/lra-all-3.pdf}
  \vspace{0.15cm}
  \caption*{\small{Fig. R2 (From LRA-paper): \textbf{Upper Table:} Results on Long-Range Arena benchmark. Best model is in boldface and second best is underlined. All models do not learn anything on Path-X task, contrary to the Pathfinder task and this is denoted by FAIL. This shows that increasing the sequence length can cause seriously difficulties for model training. The authors leave Path-X on this benchmark for future challengers but do not include it on the average (Avg.) score as it has no impact on relative performance. \textbf{Lower Table:} Benchmark results of all X-former models with a consistent batch size of 32 across all models. The authors report relative speed increase/decrease in comparison with the vanilla Transformer in brackets besides the steps per second. Memory usage refers to per device memory usage across each TPU device. Benchmarks are run on 4x4 TPU-v3 chips. \textbf{Right Fig:} Performance (y axis), speed (x axis), and memory footprint (size of the circles) of different
models.} }
  \label{fig:rebuttal_lra}
\end{figure}


==> theory_old.tex <==

\section{Theoretical convergence analysis}
\label{sec:theory}
In contrast to other methods approximating the attention matrix $\mathbf{A}$, our algorithm provides provable strong uniform convergence theoretical guarantees for compact domains. We show that $M_{\mathrm{opt}}$, the optimal number of random features, does not depend on $L$ but only on $d$. In fact, we prove that if we take $M_{\mathrm{opt}} = \Theta(d\log(d))$, then with $O(L d^2\log(d))$-time, we can approximate $\mathbf{A}$ up to any precision, regardless of the number of tokens $L$. In order to provide those guarantees for FAVOR, we leverage recent research on the theory of negative dependence for ORFs \citep{Lin2020DemystifyingOM}.
The following is true:

\begin{theorem}[Uniform convergence of FAVOR]
\label{uniform_convergence}
Take the generalized attention mechanism defined by $g,h:\mathbb{R}^{d} \rightarrow \mathbb{R}$ (see: Sec. \ref{sec:generalized}) and a radial basis function (RBF) kernel \citep{geom} $K$ with corresponding spectral distribution $\Omega$ (e.g. Gaussian kernel for which $\Omega=\mathcal{N}(0,\mathbf{I}_{d})$). Assume that the rows of matrices $\mathbf{Q}$ and $\mathbf{K}$ are taken from a ball $B(R)$ of radius $R$, centered at $0$ (i.e. norms of queries and keys are upper-bounded by $R$). 
Define $l=Rd^{-\frac{1}{4}}$ and take $g^{*} = \max_{\mathbf{x} \in B(l)}|g(\mathbf{x})|$, $h^{*} = \max_{\mathbf{x} \in B(l)}|h(\mathbf{x})|$.
Then for any $\epsilon>0$, $\delta=\frac{\epsilon}{g^{*}h^{*}}$
and the number of random features $M = \Omega(\frac{d}{\delta^{2}}\log(\frac{4\sigma R}{\delta d^{\frac{1}{4}}}))$ for $\sigma=\mathbb{E}_{\omega \sim \Omega}[\omega^{\top}\omega]$ the following holds:
$
\|\widehat{\mathbf{A}}-\mathbf{A}\|_{1} \leq \epsilon     
$
with any constant probability,
where $\widehat{\mathbf{A}}$ approximates generalized attention matrix via FAVOR with R-ORFs. 
\end{theorem}

The result holds in particular for regular attention using Gaussian kernels (see: Sec. \ref{sec:generalized}) for which $M_{\mathrm{opt}}=\Omega(\frac{d}{\delta^{2}}\log(\frac{4d^{\frac{3}{4}} R}{\delta}))$ since $\sigma = d$.



